Private Collection Matching Protocols

We introduce Private Collection Matching (PCM) problems, in which a client aims to determine whether a collection of sets owned by a server matches their interests. Existing privacy-preserving cryptographic primitives cannot solve PCM problems efficiently without harming privacy. We propose a modular framework that enables designers to build privacy-preserving PCM systems that output one bit: whether a collection of server sets matches the client's set. The communication cost of our protocols scales linearly with the size of the client's set and is independent of the number of server elements. We demonstrate the potential of our framework by designing and implementing novel solutions for two real-world PCM problems: determining whether a dataset has chemical compounds of interest, and determining whether a document collection has relevant documents. Our evaluation shows that we offer a privacy gain with respect to existing works at a reasonable communication and computation cost.

==> parts/s0-abstract.tex <==
% !TEX root = ../main.tex
\begin{abstract}
  Work on private set intersection focuses on scalability and efficiency for thin clients. These properties are essential for a number of applications, but cannot address the needs of others that involve more than one server set and require computations beyond the (cardinality of the) intersection of sets. Motivated by new settings that require many server sets and more complex computation, we propose a suite of PSI variants. The suite is based on a novel PSI primitive built on oblivious polynomial evaluation and homomorphic encryption. It is implemented as a modular framework that eases the creation of schemes to tackle new problems. We implement prototypes of concrete schemes for two real applications and empirically evaluate their performance. Our results demonstrate that our approach yields a great privacy vs. overhead trade-off.
\end{abstract}

==> resource/bfv-bench.tex <==
\begin{table}[tb]
    \centering
    \caption{Cost of basic BFV operations.}
    \begin{tabular}{lccc}
        \toprule
         & $\bfvParam{8}$ & $\bfvParam{32}$ \\ 
        \midrule
        Addition ($\mu$s)  & 29  & 530 \\     
        Multiplication (ms)  & 7.3 & 182\\   
        Plaintext mult. (ms)  & 0.97  & 18.3 \\
        Rotation by 1 (ms)  & 2.16 & 57 \\
        \midrule
        Ciphertext (KB) & 384 & 6144 \\
        Public key (KB) & 512  & 7680 \\
        Relinearization key (MB) & 3  & 60 \\
        Rotation key (MB) & 22  & 510 \\
        \bottomrule
    \end{tabular}
    \label{table:bfv-cost}
\end{table}

==> resource/bfv-param-table.tex <==
\begin{table}[tb]
    \centering
    \caption{BFV parameters with 128-bit security}
    \begin{tabular}{lcccc}
        \toprule
         & $\polyDegree$ & $\plainMod$ & $\lg(\ctxMod)$ & Mult. depth\\ 
        \midrule
        $\bfvParam{8}$ & 8192 & 4079617 &  218-bit & 2\\
        $\bfvParam{32}$ & 32768 & 786433 & 880-bit & 16\\
        \bottomrule
    \end{tabular}
    \label{table:bfv-param}
\end{table}

==> resource/doc-search.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[scale=0.55]{figures/doc_search.pdf}
    \caption{Performance evaluation of document search.}
    \label{fig:doc_eval}
  \end{figure}
  

==> resource/psi_env.tex <==
\begin{table}[tb]
    \centering
    \caption{Possible requirements and setting for PSI problems. Requirements which are supported in this work are bolded.}
    \label{table:psi-env}
    \begin{tabular*}{\columnwidth}{@{}r@{\hskip4pt}l@{}}
        \toprule
        Client's privacy & Semi-honest, \textbf{Malicious}\\ 
        Server's privacy & Semi-honest, \textbf{Malicious}\\ 
        Correctness      & \textbf{Semi-honest}, Malicious\\ 

        \hline
        Input domain & \textbf{Short (10-bit)}, \textbf{Medium (32-bit)}, \\ & Long (128-bit)\\
        Client size vs server & \textbf{Extremely unbalanced}, \textbf{Unbalanced}, \\ & Balanced\\
        Server size $(\serversize)$ & 10K, 100K, 1M, 10M, 100M, > 1B \\
        \#Server sets $(\serversetnum)$ & \textbf{Single set}, \textbf{Many-set} \\
        \hline
        Communication &  \textbf{Synchronous}, \textbf{Asynchronous}\\
        Server set & \textbf{Static}, \textbf{Infrequent changes}, \textbf{Dynamic} \\
        Pre-process com. & Per execution, One-time only, \\ & \textbf{Not needed}\\ 
        \hline

        Data transfer & For matching element, \textbf{For matching set} \\
        Gets output & \textbf{Client}, Server, Both parties \\
        \bottomrule
    \end{tabular*}
    \end{table}
    
\Kf{We need evaluation before bolding Server size in the }
